Dependent Inductive and Coinductive Types are Fibrational Dialgebras

In this paper, I establish the categorical structure necessary to interpret dependent inductive and coinductive types. It is well-known that dependent type theories \`a la Martin-L\"of can be interpreted using fibrations. Modern theorem provers, however, are based on more sophisticated type systems that allow the definition of powerful inductive dependent types (known as inductive families) and, somewhat limited, coinductive dependent types. I define a class of functors on fibrations and show how data type definitions correspond to initial and final dialgebras for these functors. This description is also a proposal of how coinductive types should be treated in type theories, as they appear here simply as dual of inductive types. Finally, I show how dependent data types correspond to algebras and coalgebras, and give the correspondence to dependent polynomial functors.

==> content/co-induction.tex <==
\section{Induction and Coinduction}
\label{sec:co-induction}

The data types definable in a data type closed category are certainly useful
but we also want to prove properties about them.
For inductive types, one usually wants to prove propositions by induction,
whereas for coinductive types the equality between elements is
important.
Both proof methods are well-understood fibrations
$L : \Cat{L} \to \Cat{D}$, where $\Cat{L}$ is to be thought of as a logic with
free variables ranging over data types in $\Cat{D}$,
see Hermida and Jacobs~\cite{HermidaJacobs-IndFib}, and
Ghani, Johann and Fumex~\cite{Ghani-IndexedInduct}.
However, the way to think about dependent types is that these
simultaneously define data types and a logic for these types, so that
we can actually construct $\Cat{L}$ for a DTCC $P : \TCat \to \BCat$.

In this section, we first construct said logic over $P$, and give a weak
induction principle within this logic that can be proved without further
assumptions.
Then we instantiate, under additional assumptions, the framework for
``fibred'' induction and coinduction, defined in~\cite{Ghani-IndexedInduct}.
It turns out that the crucial assumption is a strong elimination principle
for sums.
Next, we show that strong elimination is equivalent to dependent
recursion, where the latter seems to be a more natural requirement.
Finally, we derive a simple coinduction principle for DTCCs.

\subsection{Internal Logic}
\label{sec:int-logic}

\begin{wrapfigure}[4]{r}{.16\textwidth}
\vspace{-1.8\baselineskip}
%\hspace*{-20pt}
\begin{equation*}
  \begin{tikzcd}
    \Cat{L}
    \rar{L}
    \dar[swap]{}
    \arrow[phantom]{dr}[very near start]{\lrcorner}
    & \TCat \dar{P} \\
    \TCat
    \rar{\compr{-}}
    & \BCat
  \end{tikzcd}
\end{equation*}
\end{wrapfigure}
We begin by defining a notion of predicates $\varphi$ over data types in
a DTCC $P : \TCat \to \BCat$.
For a data type $A$, these are given as objects in
$\Cat{P}_{\compr{A}}$, that is, data types depending on $A$.
This situation is captured by the pullback (change of base) shown
on the right.
We call $L : \Cat{L} \to \Cat{E}$ the \emph{internal logic} of $P$.
Explicitly, objects in $\Cat{L}$ are pairs $(A, \varphi)$ with
$\varphi \in \Cat{P}_{\compr{A}}$ and morphisms $(A, \varphi) \to (B, \psi)$
are pairs $(f, g)$ with $f : A \to B$, $g : \varphi \to \psi$ and
$\compr{f} = Pg$.
The internal logic fibration $L$ restricts, for each $I \in \BCat$, to a
fibration $L^I : \Cat{PL}_I \to \Cat{P}_I$, where $\Cat{PL}_I$ is the fibre of
$P \circ L$ above $I$.
The reindexing functor for $u : I \to J$ is then given by
\begin{align*}
  \reidx[\#]{u}(A, \varphi)
    = (\reidx{u} A, \reidx{\compr*{\cartL{u}{A}}} \varphi)
  \qquad \reidx[\#]{u}(\id_A, f)
    = (\id_{\reidx{u} A}, \reidx{\compr*{\cartL{u}{A}}} f)
\end{align*}
where $\cartL{u}{A} : \reidx{u} A \to A$ is the cartesian lifting of $u$, see
\iDefRef{fibration}.

As seen in \iThmRef{adjunctions-from-dt}, we can define a sum
$\Sigma_{f} : \Cat{P}_I \to \Cat{P}_J$ along all $f : I \to J$ in $\BCat$ as
left adjoint to $\reidx{f}$, in other words, $P$ is
a \emph{bifibration}, see~\cite[Lem. 9.1.2]{Jacobs1999-CLTT}.
We use these sums mostly to turn a predicate over $A$
into a data type in $\Cat{P}_I$, where $I = PA$.
In this case, we use the notation $\Sigma_A \colonequals \Sigma_{\pi_A}$ for
the projection $\pi_A : \compr{A} \to I$ given in \iDefRef{CCU}.
Crucially, these projections come, by their definition, in the form of a natural
transformation $\nat{\pi}{\compr{-}}{P}$.
%, that is, for $f : A \to B$ we have $\pi_B \circ \compr{f} = P f \circ \pi_A$.
This allows us to define a fibrewise comprehension-like functor for $\Cat{L}_I$.
\begin{lemma}
  \label{lem:logic-compr}
  For each $I \in \Cat{B}$, we have the following.
  \begin{enumerate}
  \item $L^I$ is a bifibration with
    $\Sigma_{f : A \to B}(A, \varphi) = (B, \Sigma_{\compr{f}} \varphi)$.
  \item $L^I$ has a right adjoint $\K[I]{} : \Cat{P}_I \to \Cat{PL}_I$,
    given by $\K[I]{A} = (A, \K{\compr{A}})$.
  \item There is a functor $\compr{-}^I : \Cat{PL}_I \to \Cat{P}_I$, given by
    $\compr{(A, \varphi)}^I = \Sigma_{A} \varphi$, with projections
    $\nat{\pi^I}{\compr{-}^I}{L^I}$.
  \end{enumerate}
\end{lemma}
\begin{proof}
  \begin{enumerate}
  \item (Bi)fibrations are preserved under change of
    base~\cite[Lem. 1.51 and Lem. 9.1.2]{Jacobs1999-CLTT}.
  \item Fibred final objects are preserved under change of
    base~\cite[Lem 1.8.4]{Jacobs1999-CLTT}, hence we get
    $\K{} : \Cat{E} \to \Cat{L}$.
    Since it is a fibred functor, we can restrict it to
    $\K[I]{} : \Cat{P}_I \to \Cat{PL}_I$.
  \item
    To define the action of $\compr{-}^I$ on morphisms
    $(f, g) : (A, \varphi) \to (B, \psi)$, we use that
    there is a unique morphism $h : \varphi \to \reidx{\compr{f}} \psi$
    with $\cartL{\compr{f}}{\psi} \circ h = g$, where
    $\cartL{\compr{f}}{\psi} : \reidx{\compr{f}} \psi \to \psi$ is
    the cartesian morphism above $\compr{f} = Pg$, see \iDefRef{fibration}.
    Then we can put
    \begin{equation*}
      \compr{(f, g)}^I =
      \Sigma_A \varphi \xrightarrow{\Sigma_A h}
      \Sigma_A \reidx{\compr{f}} \psi \xrightarrow{\beta_\psi}
      \reidx{(Pf)} \, (\Sigma_B \psi) \cong
      \Sigma_B \psi,
    \end{equation*}
    using the canonical natural transformation
    $\beta : \Sigma_A \reidx{\compr{f}}
    \Rightarrow \reidx{P(f)} \Sigma_B$,
    which arises because $P(f) \circ \pi_A = \pi_B \circ \compr{f}$,
    and the the isomorphism coming from
    $\reidx{P(f)} = \reidx{\id_{I}} \cong \Id$.

    If $f$ and $g$ are the identity, the chosen $h$ is the identity as well,
    hence $\compr{(\id_A, \id_\varphi)}^I = \id_{\Sigma_{A} \varphi}$.
    To show that
    $\compr{(f_2, g_2) \circ (f_1, g_1)}^I =
    \compr{(f_2, g_2)}^I \circ \compr{(f_1, g_1)}^I$,
    one uses that $\beta$ is natural, the coherence conditions of a cloven
    fibration and the fact that the chosen $h_1$ and $h_2$ for $g_1$ and
    $g_2$, respectively, compose.

    The projections are obtained as follows.
    For each $A$, we can define a morphism
    $\mathrm{prj}_A : \T_{\compr{A}} \to \reidx{\pi_A} A$ as the unique map
    mediating the counit $\varepsilon_A : \T_{\compr{A}} \to A$ of
    $\T \dashv \compr{-}$ and the Cartesian lifting
    $\cartL{\pi_A}{A} : \reidx{\pi_A} A \to A$.
    This gives a map
    $\varphi \xrightarrow{!_\varphi}
    \T_{\compr{A}} \xrightarrow{\mathrm{prj}_{A}} \reidx{\pi_A} A$,
    hence a unique morphism $\pi^I_\varphi : \Sigma_A \varphi \to A$.
    Naturality of $\pi^I$ follows.
    \qedhere
  \end{enumerate}
\end{proof}

\subsection{Induction and Dependent Recursion}
\label{sec:dep-rec}

We are now going to study dependent recursion and induction principles for
inductive data types in the scene set above.

First, we derive a weak dependent recursion principle that can be defined
in any DTCC.
The idea is that we can track dependencies using sums, that is, given
$(A, \varphi) \in \Cat{PL}_I$, we can pack this predicate to
$\compr{(A, \varphi)}^I = \Sigma_A \varphi \in \Cat{P}_I$.
\begin{proposition}
  \label{prop:weak-induction}
  Let $(F, u)$ be a signature with $F : \Cat{P}_I \to \Cat{C}$,
  $(A, \alpha)$ an initial $(F, G_u)$-dialgebra,
  and $d : F \compr{(A, \varphi)}^I \to G_u \compr{(A, \varphi)}^I$, such that
  $\pi^I_\varphi : \compr{(A, \varphi)}^I \to A$ is a homomorphism.
  Then there is a unique homomorphism
  $h : (A,\alpha) \to (\compr{(A, \varphi)}^I, d)$ with
  $\pi^I_\varphi \circ h = \id_A$.
\end{proposition}
\begin{proof}
  The homomorphism $h$ is the inductive extension of $d$ and,
  since $\pi^I_\varphi \circ h$ is an endomorphism on $\alpha$, it must be the
  identity by uniqueness of inductive extensions.
\end{proof}

\begin{example}
  Recall that we defined vectors as the initial $(F, G_u)$-dialgebra with
  $F = \prodArr{\T, K_A \times \Id}$ and $G_u = \prodArr{\reidx{z}, \reidx{s}}$,
  giving rise to the constructor $\alpha = (\nil, \cons)$.
  In this case, the condition on $d = (d_1, d_2)$ becomes
  \begin{align*}
    & d_1 : \T \to \reidx{z}(\Sigma_{\VecT A}(\varphi))
    && \reidx{z}(\pi^I_\varphi) \circ d_1 = \nil \\
    & d_2 : A \times \Sigma_{\VecT A}(\varphi)
      \to \reidx{s}(\Sigma_{\VecT A} (\varphi))
    && \reidx{s}(\pi^I_\varphi) \circ d_2
    = \cons \circ \, (\id_A \times \pi^I_\varphi),
  \end{align*}
  which is, modulo the use of sums, the usual condition for induction
  base and step.
  \qed
\end{example}

\propRef{weak-induction} allows us to prove predicates on an initial dialgebra,
this approach has, however, two shortcomings.
First, we can use the principle only on initial dialgebras, since we
otherwise cannot construct the homomorphism with the required property.
Secondly, the result of the induction is buried under a sum, hence we can use
the result of an induction only in (non-dependent) recursion.
Both problems can be fixed if we assume strong sums.

We say that $P$ has \emph{strong sums}, if the dependent pairing
$\kappa : \compr{\varphi} \to \compr{\Sigma_A \varphi}$ has an inverse, where
$\kappa = \compr{\cartL{\pi_A}{(\Sigma_A \varphi)} \, \circ \, \eta_{\varphi}}$
and $\nat{\eta}{\Id}{\reidx{\pi_A} \Sigma_A}$.
This allows us to prove the following lemma, which is key to derive an induction
principle.
\begin{lemma}
  \label{lem:adjoint-from-strong-sum}
  If $P$ admits strong sums and full comprehension, then
  $K^I \dashv \compr{-}^I$.
\end{lemma}
\begin{proof}
  The crucial point is that we need strong elimination
  $\Sigma_A \varphi \to \varphi$ to define the counit of
  $K^I \dashv \compr{-}^I$.
  We leave the details of the verification out.
\end{proof}
Combining \iLemRef{adjoint-from-strong-sum} and a variation of
\cite[Cor. 6.6]{Ghani-IndexedInduct}, we get an induction principle on the
the algebras arising from data types, see~\iThmRef{iso-dialg-alg}, under the
assumption that sums in $\TCat$ are strong.
Note that we, in contrast to~\cite{Ghani-IndexedInduct}, only have comprehension
on fibres $\Cat{P}_I$ available, since we cannot define the action on morphisms
on all of $\TCat$.
This is, however, not a necessary requirement to carry out the proofs in
loc.~cit.

Let us briefly discuss how strong sums arise in the type system of Agda.
The commonly used definition of sums ($\Sigma$-types) is the following.
\begin{center}
\begin{lstlisting}[language=Agda,mathescape=true,columns=flexible]
record $\Sigma$ (A : Set) (B : A $\to$ Set) : Set where
  p$_1$ : A
  p$_2$ : B p$_1$
\end{lstlisting}
\end{center}
Note that the second destructor refers to the first, which is not allowed in
our setup and leads to a strong elimination principle for $\Sigma$.
Our definition actually corresponds to
\begin{center}
\begin{lstlisting}[language=Agda,mathescape=true,columns=flexible]
data $\Sigma'$ (A : Set) (B : A $\to$ Set) : Set where
  in : (a : A) $\to$ B a $\to$ $\Sigma'$ A B
\end{lstlisting}
\end{center}
for which we can only define $\mathrm{fst}_B : \Sigma' \, A \, B \to A$,
corresponding to the $\pi^I_B$ we defined above.
If we were to have a dependent recursion principle
\begin{equation*}
  \AxiomC{$\typed[x : A, y : B \, x]{f}{C \, (\mathrm{in} \, x \, y)}$}
  \UnaryInfC{$\typed[z : \Sigma \, A \, B]{\rec f}{C z}$}
  \DisplayProof
\end{equation*}
then we could, in fact, derive strong elimination by using
$C = \reidx{\mathrm{fst}_B}(B)$ and $f = y$.

This leaves us with the question of how dependent elimination can be defined
using dialgebras, i.e., how far can we go without using strong elimination of
sums, but rather derive it?
As a start, we restate the result in~\cite[Thm. 4.14]{Ghani-GenericInduction}
under weaker conditions, namely without using the full adjunction
$\K[I]{} \dashv \compr{-}^I$.
\begin{lemma}
  \label{lem:lift-parts}
  If $P : \Cat{E} \to \Cat{B}$ is a DTCC, then there is a functor
  $\mathcal{L}^I : \Cat{PL}_I \to \ArrC{\Cat{P}_I}$
  given by
  $\mathcal{L}^I(A, \varphi) = \pi^I_\varphi : \Sigma_A \varphi \to A$,
  and a functor $U^I : \ArrC{\Cat{P}_I} \to \Cat{PL}_I$.
  Moreover, $U^I$ preserves final objects and, if $P$ has full comprehension,
  then $\mathcal{L}^I$ preserves final objects as well.
\end{lemma}
\begin{proof}
  Functoriality of $\mathcal{L}^I$ follows readily from $\pi^I$ being
  a natural transformation.
  $U^I$ is given, as in~\cite{Ghani-GenericInduction}, by
  \begin{equation*}
    U^I(f : A \to B)
    = \Sigma^I_f(\KI{A})
    = \Sigma^I_f(A, \K{\compr{A}})
    = (B, \Sigma_{\compr{f}}\K{\compr{A}}).
  \end{equation*}
  The definition of $U^I$ on morphisms is slightly more complicated,
  see loc.~cit., we note however that it only uses properties of cartesian
  liftings.

  The proof that $U^I$ preserves final objects is given by
  Ghani et al.~\cite[Thm. 4.14]{Ghani-GenericInduction}.
  That $\mathcal{L}^I$ preserves terminal objects
  means that it maps $\cramped{\K[I]{A} = \left(A, \K{\compr{A}}\right)}$ to an
  isomorphism.
  This is indeed the case here, as, by fullness, the map
  $\mathrm{\pi}^I_\varphi : \Sigma_A \K{\compr{A}} \to A$ is an isomorphism,
  see~\cite[Ex. 10.5.4]{Jacobs1999-CLTT}.
  The rest of the proof in~\cite{Ghani-GenericInduction} can be preserved.
\end{proof}

As in~\cite{Ghani-IndexedInduct}, we can combine these functors into
a lifting of functors $F : \Cat{P}_I \to \Cat{P}_J$ to
functors $\liftF{F} : \Cat{PL}_I \to \Cat{PL}_J$ by putting
$\liftF{F} = R^J \ArrC{F} \mathcal{L}^I$,
where $\ArrC{F} : \ArrC{\Cat{P}_I} \to \ArrC{\Cat{P}_J}$ is given by
$\ArrC{F}(f : A \to B) = Ff : FA \to FB$.
This allows us to lift a signature
$(F, G) : \Cat{P}_I \to \prod_{k=1,\dotsc,n} \Cat{P}_{J_k}$ with
$G = \prodArr{\reidx{u_1}, \dotsc, \reidx{u_n}}$ to a signature
$(\liftF{F}, \liftF{G}) : \Cat{PL}_I \to \prod_{k=1,\dotsc,n} \Cat{PL}_{J_k}$,
by putting $\liftF{F}_k = R^{J_k} \ArrC{F_k} \mathcal{L}^I$ and
$\liftF{G}_k = \reidx[\#]{u_k}$.
The liftings $\liftF{F}$ and $\liftF{G}$ preserve fibred final objects by
\iLemRef{lift-parts} and by reindexing preserving fibred structure,
respectively.
Hence they are \emph{truth-preserving}, in the sense that
$\liftF{F} \circ \K[I]{} \cong
\left(\prod_{k=1,\dotsc,n} \K[J_k]{}\right) \circ F$ and the same for
$\liftF{G}$.

Let us now analyse what dialgebras for these lifted functors are.
Recall that a morphism $r : \liftF{F}(A, \varphi) \to \liftF{G}(A, \varphi)$ in
is in fact an $n$-tuple of pairs $((d_1, b_2), \dotsc, (d_n, b_n))$,
such that $(d_1, \dotsc, d_n) : FA \to GA$ is an $(F, G)$-dialgebra,
$b_k : \Sigma_{\compr{F_k \pi^I_\varphi}} \K[J_k]{F_k \compr{\varphi}^I}
\to \reidx{\compr{\cartL{u_k}{A}}}\varphi$
and $\compr{d_k} = P(b_k)$.
If $A \in \SetC^I$ and $\varphi \in \SetC^{\coprod_{i \in I} A_i}$, then we have
$\compr{\varphi}^I(i \in I) = \coprod_{x \in A(i)} \varphi(i, x)$, and for
each $j \in J_k$ and $x \in F_k A$  the components of $b_k$ are of the form
\begin{equation*}
  b_k(j, x) :
    \smashoperator[r]{
      \coprod_{\substack{u \, \in \, F_k(\compr{\varphi}^I)(j) \\
          F_k(\pi^I_{\varphi}) \, u = x}}
    } \; \T(j, u)
      \to \varphi(u_k \, j, d_k \, x).
\end{equation*}
Most importantly, note the use of $d_k$ in the codomain of $b_k$.

The intuition is that each $b_k$ proves that, from the induction hypothesis that
$\varphi$ holds at the argument of the constructor $d_k$, $\varphi$ holds
at $d_k \, x$.
For example, let $A = \VecT B$,  $F_2 = B \times \Id$, $u_2 = s$, and
$d_2 = \cons$.
Then the assumption of $b_2(k, (a \in A, v \in \VecT B \, k))$ boils down to
a proof of $\varphi \, k \, v$, and the conclusion of $b_2$ is that
$\varphi$ holds at $k+1$ and $\cons_k (a, v)$.

To explain dependent recursion, we define
$\DialgC[F,G]{\T} : \DialgC{F,G} \to \DialgC{\liftF{F}, \liftF{G}}$ by
mapping a dialgebra $d : FX \to GX$ to a dialgebra
$d' : \liftF{F}\left( \K[I]{X} \right) \to \liftF{G} \left( \K[I]{X} \right)$,
using that the liftings are truth-preserving.
If we now require that $\DialgC[F,G]{\T}$
preserves initial dialgebras (cf.~\cite{HermidaJacobs-IndFib}), we get
dependent recursion for $A = \mu (F, G)$, as there is then a unique homomorphism
$(\id_A,h) : (A, \K{\compr{A}}) \to (A, \varphi)$, i.e.,
for each $k$, $i \in I$ and $x \in A$, a map $h_k(i, x) : \T \to \varphi(i, x)$.
This allows us, since $\T$ is final, to canonically construct an element
of $\varphi$ for each $i$ and $x$.
In other words, we can carry out dependent recursion on $A = \mu (F, G)$,
and prove predicates by induction.
Combining this with the derivation of strong sum elimination from dependent
recursion and \iLemRef{adjoint-from-strong-sum}, we have the following
result.
\begin{corollary}
  A data type closed category admits dependent recursion, hence induction,
  iff it has strong sums.
\end{corollary}

% \subsection{Induction -- A Summoning Ritual in 7 steps}
% \label{sec:induction}

% that arises from a comprehension category
% $\mathcal{P} : \TCat \to \ArrC{\BCat}$ as $p = \cod \circ \, \mathcal{P}$.
% This gives us, as usual, the comprehension functor
% $\compr{-} = \dom \circ \, \mathcal{P}$.

% \begin{enumerate}
% \item Define truth functor $K : \BCat \to \TCat$ by
%   $K(I) = \T_I = \nu (\reidx{\id}, \Id)$, see \iExRef{dt-complete}.
% \item \red{Require} that $K \dashv \compr{-}$.
% \item Given a data signature
%   $F, G : \Cat{P}_I \to \prod_{k=1,\dotsc,n} \Cat{P}_{J_k}$, we put
%   $A = \mu(F, G)$ and define liftings
%   $\liftF{F}, \liftF{G} : \Cat{P}_{\compr{A}} \to
%   \prod_{k=1, \dotsc, n} \Cat{P}_{\compr{F_k A}}$.
% \item Define \emph{pseudo-induction}: From the recursion on
%   $\top_A = \mu(\liftF{F}, \liftF{G}) \in \Cat{P}_{\compr{A}}$, we get for each
%   $L \in \Cat{P}_{\compr{A}}$ and a dialgebra
%   $a : \liftF{F}(L) \to \liftF{G}(L)$ a pseudo-proof $u : \top_A \to L$.
% \item \red{Require} that there is a
%   $\true_A : \compr{A} \to \compr{\top_A}$, which is a section for
%   $\mathcal{P}(\top_A) = \pi_{\top_A} : \compr{\top_A} \to \compr{A}$,
%   that is, $\pi_{\top_A} \circ \true_A = \id_{\compr{A}}$.
% \item Use adjunction $K \dashv \compr{-}$
%   \begin{equation*}
%     \begin{adjunction}
%       \true_A : & \compr{A} & \compr{\top_A} & \text{in } \BCat \\ \hhline{====}
%       \widecheck{\true_A} : & K(\compr{A}) & \top_A
%       & \text{in } \Cat{P}_{\compr{A}}
%     \end{adjunction}
%   \end{equation*}
%   and note that $\T_{\compr{A}} = K(\compr{A})$.
% \item \emph{Induction} follows by composition:
%   $\T_{\compr{A}} \xrightarrow{\widecheck{\true_A}} \top_A \xrightarrow{u} L$.
% \end{enumerate}

\subsection{Coinduction}
\label{sec:coind}

As observed by Hermida and Jacbos~\cite{HermidaJacobs-IndFib}, coinduction is
concerned with relations that witness the equality between elements of
coinductive types.
We show here how to establish a simple form of coinduction on elements of final
dialgebras.

\begin{wrapfigure}[4]{r}{.22\textwidth}
\vspace{-1.8\baselineskip}
%\hspace*{-20pt}
\begin{equation*}
  \begin{tikzcd}[column sep=0.5cm]
    \Rel{\Cat{P}_I}
    \rar{}
    \dar[swap]{} %{R^I}
    \pullback
    & \Cat{PL}_I \dar{L^I} \\
    \Cat{P}_I
    \rar{\Delta}
    & \Cat{P}_I
  \end{tikzcd}
\end{equation*}
\end{wrapfigure}
We first define relations internal to a data type closed category.
Such relations are given as objects in the pullback, displayed on the right,
of $L^I$ along $\Delta$ with $\Delta(A) = A \times_I A$.
Let us abbreviate $A \times_I A$ to $A^2$ in the following.
The representation of $\Rel{\Cat{P}_I}$, we will use, has objects $(A, R)$
with $PR = \compr{A^2}$ and morphisms
$(f, g) : (A, R) \to (A', R')$ with $f : A \to A'$,
$g : R \to R'$ and $Pg = \compr{f \times_I f}$.

\begin{wrapfigure}[5]{l}{.4\textwidth}
  \vspace{-1.8\baselineskip}
  % \hspace*{-20pt}
  \begin{equation*}
    \begin{tikzcd}[column sep=1.5cm]
      G_u(Q(A,R)) \dar{d} \rar{\nabla^{G_u} \circ G_u(\pi^I_{R})}
      & G_u(A)^2 \dar{\outNu \times_I \outNu} \\
      F(Q(A,R)) \rar{\nabla^F \circ F(\pi^I_{R})}
      & F(A)^2
    \end{tikzcd}
  \end{equation*}
\end{wrapfigure}
Within this setup, we can define a (quotient-like) functor $Q : \Rel{\Cat{P}_I} \to \Cat{P}_I$
by $Q(A, R) = \Sigma_{A^2} R = \compr{(A^2, R)}^I$.
Let $\nat{\delta}{\Id_{\Cat{P}_I}}{\Delta}$ be the diagonal and
$\nabla^H : H(A^2) \to H(A) \times_I H(A)$ the canonical morphism.
Then we can derive the following coinduction principle.
\begin{proposition}
  Let $(F, u)$ be a signature with $F : \Cat{P}_I \to \Cat{C}$,
  $(A, \outNu)$ a final $(G_u, F)$-dialgebra,
  $(A, R) \in \Rel{\Cat{P}_I}$ and
  $d : G_u(Q(A, R)) \to F(Q(A, R))$, such that
  the diagram on the left commutes.
  Then there is a unique $h : Q(A, R) \to A$ with
  $\delta_A \circ h = \pi^I_R$.
\end{proposition}
\begin{proof}
  By definition, we have for $i =1,2$ that
  $\pi_i \circ \nabla^{G_u} = G_u(\pi_i)$,
  hence we find
  $\pi_i \circ \nabla^{G_u} \circ G_u(\pi^I_R) = G_u(\pi_i \circ \pi^I_R)$,
  and the same for $F$.
  Thus $\pi_i \circ \pi^I_{R}$ is a homomorphism from $d$ to $\outNu$ and
  must therefore be equal to $h$.
  Since this holds for $i=1,2$, we have $\pi^I_R = \delta_A \circ h$.
\end{proof}

\begin{example}
  Let $F = \prodArr{K_A, \Id}$ and
  $u = (\id_\T, \id_\T)$, so that streams $\Str{A}$ are
  given by $\nu (G_u, F)$ with
  $(\head, \tail) : G_u(\Str{A}) \to F(\Str{A})$.
  The conditions for a dialgebra
  $G_u(\Sigma_{\Str{A} \times \Str{A}}(R)) \to
  (A, \Sigma_{\Str{A} \times \Str{A}}(R))$
  over a relation $R$ on $\Str{A}$ then capture the usual
  bisimulation proof principle.
  % $(d_1, d_2)$ with $d_1 : \Sigma_{\Str{A} \times \Str{A}}(R) \to A$
  % and
  % $d_2 : \Sigma_{\Str{A} \times \Str{A}}(R) \to
  % \Sigma_{\Str{A} \times \Str{A}}(R)$,
  % then the condition reads as
  % $\delta \circ d_1 = \head \circ \, \pi_{R}$
  % and $\pi_R \circ d_2 = (\tail \times \tail) \circ \pi_R$.
\end{example}

This coinduction principle suffers again from the problem that it cannot be
applied to arbitrary dialgebras.
Moreover, we can use it to prove functions to be equal, by proving that they
agree on every argument.
Hence, in an intensional type theory, the requirement to have final dialgebras
must be relaxed to weakly final dialgebras.
In that case, we like would to still be able to give a canonical notion of,
for example, bisimulation. %, just as we have done in \iExRef{dt-complete}.
Ghani et al.~\cite{Ghani-IndexedInduct} have defined a canonical lifting
of functors to relations, but this lifting process relies on having a quotient
functor, and there does not seem to be a way out of this, like for the liftings
we used for induction.
Thus we leave the question of how to describe coinduction open for now.


%%% Local Variables:
%%% TeX-master: "../FibDialg-CALCO"
%%% ispell-local-dictionary: "british"
%%% mode: latex
%%% End:

==> content/dt-bc-cond.tex <==
\section{Beck-Chevalley Condition for Data Types}
\label{sec:b-c-cond}

When dealing with dependent types, we find ourselves often in the situation
that we want to change the index of a type through substitutions but
still preserve the structure of said type.
For example, we constructed vectors indexed by \emph{some} representation
of natural numbers, but there is no reason that the definition
behaves the same among all choices.
Thus, we would like to force that, for example, vectors indexed by the
canonical representation of natural numbers and those indexed by, say,
lists over $\T$ are essentially the same.
We formally capture this by the Beck-Chevalley condition, proposed below.
The name comes from a condition that is usually imposed on dependent products
and coproducts to ensure that these are stable under reindexing.
The relation is established in \iThmRef{fibred-adjunction-bc-cond}.

% We have seen vectors as data type indexed by natural numbers, however,
% we did not specify 



% \begin{wrapfigure}[4]{r}{.15\textwidth}
% \vspace{-1.8\baselineskip}
% %\hspace*{-20pt}
% \begin{equation*}
%   \begin{tikzcd}
%     L \rar{u} \dar[swap]{g}
%     \arrow[phantom]{dr}[very near start]{\lrcorner}
%     & I \dar{f} \\
%     K \rar{v}
%     & J
%   \end{tikzcd}
% \end{equation*}
% \end{wrapfigure}
% A common condition imposed on (co)products is the
% \emph{Beck-Chevalley condition}, defined as follows.
% If we are given a pullback square in $\Cat{B}$, as displayed on the right,
% then there is a canonical natural transformation
% $\reidx{v} \prod_f \Rightarrow \prod_g \reidx{u}$.
% The Beck-Chevalley condition for the product requires this to be an
% isomorphism.
% We now define a similar condition on data types in general.

Let $(F, G)$ be a signature with $F : \Cat{C} \times \Cat{P}_I \to \Cat{D}$,
$G = \prodArr{\reidx{u_1}, \dotsc, \reidx{u_n}}$ and $u_i : J_i \to I$.
Assume that we are given for each $1 \leq i \leq n$ a pullback square
\begin{equation}
  \label{eq:dt-pb}
  \begin{tikzcd}
    L_i \rar{w_1} \dar[swap]{x_i}
    \pullback
    & J_i \dar{u_i} \\
    K \rar{v}
    & I
  \end{tikzcd}
\end{equation}
Then there are isomorphisms
$\iota^{G,i} : \reidx{x_i} \circ \reidx{v}
% \cong \reidx{(v \circ x_i)} = \reidx{(u_i \circ w_i)}
\cong \reidx{w_i} \circ \reidx{u_i}$,
since $P$ is a cloven fibration.
This gives us functors $G^v : \Cat{P}_K \to \prod_{i=1}^n \Cat{P}_{L_i}$
with $G^v = \prodArr{\reidx{x_1}, \dotsc, \reidx{x_n}}$
and $W : \prod_{i=1}^n \Cat{P}_{J_i} \to \Cat{P}_{L_i}$
with $W = \reidx{w_1} \times \dotsm \times \reidx{w_n}$, and an isomorphism
$\iota^G : G^v \reidx{v} \cong W G$.

Let us, moreover, assume that there is a functor
$F^v : \Cat{C} \times \Cat{P}_K \to \prod_{i=1}^n \Cat{P}_{L_i}$ and
an isomorphism $\nat{\iota^F}{F^v (\Id \times \reidx{v})}{W F}$
as indicated in the following diagram.
\begin{equation*}
  \begin{tikzcd}
    \Cat{C} \times \Cat{P}_I
      \rar{F}
      \dar[swap]{\Id \times \reidx{v}}
    & \prod_{i=1}^n \Cat{P}_{J_i} = \Cat{D}
      \dar{W} \\
    \Cat{C} \times \Cat{P}_K
      \rar{F^v}
      \arrow[Rightarrow]{ur}{\cong}
    & \prod_{i=1}^n \Cat{P}_{L_i}
  \end{tikzcd}
\end{equation*}
Using this data, we can define a functor
$\PBCoind{v} : \DialgC{\funCur{G}, \funCur{F}}
\to \DialgC{\funCur{G^v}, \funCur{F^v}}$
as follows.
Let $\nat{\delta}{\funCur{G}(H)}{\funCur{F}(H)}$ be a dialgebra, then
$\PBCoind{v}(\delta)$ is the composition
\begin{align*}
  \funCur{G^v}(\reidx{v} H)
  & = G^v \reidx{v} H \\
  & \xRightarrow{\iota^GH} W G H
  = W \funCur{G}(H) \\
  & \xRightarrow{W \delta} W \funCur{F}(H)
  = W F \prodArr{\Id_\Cat{C}, H} \\
  & \xRightarrow{\left(\iota^F\right)^{-1} \prodArr{\Id_\Cat{C}, H}}
    F^v (\Id_{\Cat{C}} \times \reidx{v}) \prodArr{\Id_\Cat{C}, H}
  = F^v \prodArr{\Id_\Cat{C}, \reidx{v} H}
  = \funCur{F^v}(\reidx{v} H).
\end{align*}
For a dialgebra homomorphism $\nat{\beta}{H_1}{H_2}$ from $\delta_1$ to
$\delta_2$, we put $\PBCoind{v}(\beta) = \reidx{v} \beta$, which is a
$(\funCur{G^v}, \funCur{F^v})$-dialgebra homomorphism since the following
diagram commutes.
\begin{equation*}
  \begin{tikzcd}[every arrow/.style={draw, Rightarrow}, column sep = 2cm]
    \funCur{G^v}(\reidx{v} H_1)
      \rar{\funCur{G^v}(\reidx{v}\beta)}
      \dar[swap]{\iota^G H_1}
      \arrow[phantom]{dr}{\iota^G \text{ nat. }}
    & \funCur{G^v}(\reidx{v} H_2)
      \dar{\iota^G H_2} \\
    W \funCur{G}(H_1)
      \rar{W \funCur{G}(\beta)}
      \dar[swap]{W \delta_1}
      \arrow[phantom]{dr}{\beta \text{ hom. }}
    & W \funCur{G}(H_2)
      \dar{W \delta_2} \\
    W \funCur{F}(H_1)
      \rar{W \funCur{F}(\beta)}
      \dar[swap]{(\iota^F)^{-1} \prodArr{\Id, H_1}}
      \arrow[phantom]{dr}{\iota^F \text{ nat. }}
    & W \funCur{F}(H_2)
      \dar{(\iota^F)^{-1} \prodArr{\Id, H_2}} \\
    \funCur{F^v}(\reidx{v} H_1)
      \rar{\funCur{F^v}(\reidx{v} \beta)}
    & \funCur{F^v}(\reidx{v} H_2)
  \end{tikzcd}
\end{equation*}
The functor laws for $\PBCoind{v}$ follow from functoriality of $\reidx{v}$.
Dually, we can define a functor
$\PBInd{v} : \DialgC{\funCur{F}, \funCur{G}} \to
  \DialgC{\funCur{F^v}, \funCur{G^v}}$
by
\begin{align*}
  & \PBInd{v}(\nat{\delta}{\funCur{F}(H)}{\funCur{G}(H)})
    = (\iota^G)^{-1}H \circ W \delta \circ \iota^F \prodArr{\Id_\Cat{C}, H} \\
  & \PBInd{v}(\beta) = \reidx{v} \beta.
\end{align*}
These functors allow us to define what it means that data types are preserved by
reindexing.
\begin{definition}
  A coinductive data type $(\Omega, \xi)$ for $(F, G)$ fulfils the
  \emph{Beck-Chevalley condition}, if for every family of pullbacks
  $\PB[I]{v}{u_i}$ as in \eqRef{dt-pb}, there is a functor $F^v$ and an
  isomorphism $\iota^F$ as described above, such that  the coinductive
  extension of $\PBCoind{v}(\xi)$ to the the CDT $(\Omega^v, \xi^v)$ for
  $(F^v, G^v)$, is an isomorphism
  $\PBCoind{v}(\xi) \cong \xi^v$.
  The Beck-Chevalley condition for IDTs is defined dually using $\PBInd{v}$.
\end{definition}

As the name suggests, this definition is supposed to capture the
known Beck-Chevalley conditions.
To prove this, we need the following result.
\begin{lemma}
  \label{lem:left-distr-mu-comp}
  Let $F_1 : \Cat{C}_1 \to \Cat{C}_2$ be a functor and
  $(F_2 : \Cat{C}_2 \times \Cat{P}_I \to \Cat{C}_3, G)$ be a signature.
  If we define
  $F = F_2 \circ (F_1 \times \Id) :
    \Cat{C}_1 \times \Cat{P}_I \to \Cat{C}_3$,
  then
  $\mu (\funCur{F}, \funCur{G}) = \mu(\funCur{F_2}, \funCur{G}) \circ F_1$ and
  $\alpha^{(\funCur{F}, \funCur{G})} = \alpha^{(\funCur{F_2}, \funCur{G})} F_1$.
  Dually, we have that
  $\nu(\funCur{G}, \funCur{F}) = \nu(\funCur{G}, \funCur{F_2}) \circ F_1$ and
  $\xi^{(\funCur{F}, \funCur{G})} = \xi^{(\funCur{F_2}, \funCur{G})} F_1$.
\end{lemma}
\begin{proof}
  This follows simply from the definitions.
  Let $V \in \Cat{C}_1$, then
  \begin{align*}
    \mu (\funCur{F}, \funCur{G})(V)
    & = \mu (F(V, -), G)
    = \mu ((F_2 \circ (F_1 \times \Id))(V, -), G)
    = \mu (F_2(F_1(V), -), G) \\
    & = \mu (\funCur{F_2}, \funCur{G})(F_1(V))
    = (\mu (\funCur{F_2}, \funCur{G}) \circ F_1)(V)
  \end{align*}
  and the equality of the natural transformations follows immediately from
  their definition and the functor equality above.
  \qedhere
\end{proof}

Let us come back to the example we mentioned in the beginning.
\begin{example}
  Recall that we have used \emph{some} object $\N$ as index for vectors that
  has maps $z : \T \to \N$ and $s : \N \to \N$.
  The obvious choice to construct $\N$ is of course as
  $\mu (\prodArr{K_\T, \Id}, \Delta)$ with
  $\Delta = \prodArr{\reidx{\id_\T}, \reidx{\id_\T}}$,
  which just captures exactly these constructors.
  However, we can also consider lists over $\T$, with constructors
  $\nil : \T \to \List{\T}$ for the empty list and
  $\ast \coloncolon (-) : \List{\T} \to \List{\T}$ for prefixing with $\ast$.
  Then there is an isomorphism $g : \List{\T} \to \N$ of
  $(\prodArr{K_\T, \Id}, \Delta)$-dialgebras.
  From here, we can derive two pullbacks $(\nil, \id_\T) = g \times_\N z$ and
  $(\ast \coloncolon (-), g) = g \times_\N s$.
  Then Beck-Chevalley condition then demands that
  $\reidx{g}(\VecT A) \cong \mu (F, G)$ for the functors
  $F = \prodArr{K_\T, K_{\reidx{g}(A)} \times \Id}$ and
  $G = \prodArr{\reidx{\nil}, \reidx{(\ast : (-))}}$.

  % with constructors
  % $z : \T \to \N$ and $s : \N \to \N$.
  % Likewise, lists $\List{A}$ over $A$ with constructors
  % $\nil$ and $\_:\_$ are an initial
  % $(\prodArr{K_\T, K_A \times \Id},
  % \prodArr{\reidx{\id_\T}, \reidx{\id_\T}})$-dialgebra.
  % Since $\T \times X \cong X$ for any $X$, we have $\List{\T} \cong \N$ as
  % dialgebras.
  % This gives us the two pullbacks
  % \begin{equation*}
  %   \begin{tikzcd}
  %     \T
  %     \rar{\id} \dar[swap]{\nil}
  %     \pullback
  %     & \T \dar{z} \\
  %     \List{\T} \rar{g} & \N
  %   \end{tikzcd}
  %   \qquad
  %   \begin{tikzcd}
  %     \List{\T}
  %     \rar{g} \dar[swap]{\ast : (-)}
  %     \pullback
  %     & \N \dar{s} \\
  %     \List{\T} \rar{g} & \N
  %   \end{tikzcd}
  % \end{equation*}
  % and we find $\reidx{g}(\VecT A) \cong \mu (F, G)$ where
  % $F = \prodArr{K_\T, K_{\reidx{g}(A)} \times \Id}$ and
  % $G = \prodArr{\reidx{\nil}, \reidx{(\ast : (-))}}$.
\end{example}


Now we can show the usual B-C condition and our version
for data types to be equivalent.
\begin{theorem}
  \label{thm:fibred-adjunction-bc-cond}
  The adjunctions constructed in \iThmRef{adjunctions-from-dt} are fibred iff
  they fulfil the Beck-Chevalley condition for data types.
\end{theorem}
\begin{proof}
  We prove this for the constructed right adjoints, the proof for the left
  adjoints follows by duality.
  Recall that we defined for $\Cat{C} = \prod_{i=1}^n \Cat{P}_{J_i}$,
  a right adjoint for all
  $G = \prodArr{\reidx{u_1}, \dotsc, \reidx{u_n}}$ by
  $\nu (\funCur{G}, \funCur{\pi_1}) : \Cat{D} \to \Cat{P}_I$ with
  $\pi_1  : \Cat{C} \times \Cat{P}_I \to \Cat{C}$.
  Given pullbacks $(x_i, w_i) = \PB[I]{v}{u_i}$ as in \eqRef{dt-pb}, we put
  $\Cat{D} = \prod_{i=1}^n \Cat{P}_{L_i}$, $W : \Cat{C} \to \Cat{D}$
  with $W = \reidx{w_1} \times \dotsm \times \reidx{w_1}$ and
  $G^v = \prodArr{\reidx{x_1}, \dotsc, \reidx{x_n}}$.
  We find the right adjoint of $G^v$ to be $\nu (\funCur{G^v}, \funCur{\pi_1'})$
  with $\pi_1' : \Cat{D} \times \Cat{P}_K \to \Cat{D}$.

  The Beck-Chevalley condition for adjoints requires that the canonical
  natural transformation
  $\gamma : \reidx{v} \circ \nu (\funCur{G}, \funCur{\pi_1})
  \Rightarrow \nu (\funCur{G^v}, \funCur{\pi_1'}) \circ W$
  is an isomorphism.
  We show that this coincides with our definition for data types.

  Let $\xi$ be the final $(\funCur{G}, \funCur{\pi_1})$-dialgebra
  and $\xi^v$ the final $(\funCur{G^v}, \funCur{F^v})$-dialgebra.
  We note that $\pi_1' \circ (W \times \Id) = W \pi_1''$, where
  $\pi_1'' : \Cat{C} \times \Cat{P}_K \to \Cat{C}$.
  Thus, we can choose for the B-C condition $F^v = W \pi_1''$ and
  get, by \iLemRef{left-distr-mu-comp},
  $\nu (\funCur{G^v}, \funCur{F^v})
  = \nu (\funCur{G^v}, \funCur{\pi_1'}) \circ W$.
  By finality, this means that $\gamma$ is in fact the unique morphism
  from $\PBCoind{v}(\xi)$ to $\xi^v$.
  The B-C condition for data types requires this to be an isomorphism,
  just as the B-C condition for adjoints does.
  This means that the constructed adjunctions are fibred iff
  they satisfy the B-C condition for data types with the choice
  $F^v = W\pi_1''$.
  \qedhere
\end{proof}

In the same way, we can relate fibred final objects and the B-C condition.
\begin{theorem}
  Terminal objects $\T_I$, constructed as
  $\nu (\reidx{\id_I}, \Id_{\Cat{P}_I})$, are fibred iff they satisfy the
  Beck-Chevalley condition for data types.
\end{theorem}
\begin{proof}
  We note that the pullback \eqRef{dt-pb} degenerates, in this case, to only
  give a morphism $v : K \to I$.
  Then we pick $\Id^v = \reidx{v}$ and the rest follows as in
  \iThmRef{fibred-adjunction-bc-cond}.
  \qedhere
\end{proof}

%%% Local Variables:
%%% TeX-master: "../FibDialg-CALCO"
%%% ispell-local-dictionary: "british"
%%% mode: latex
%%% End:

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{R. Matthes, M. Mio (Eds.): Fixed Points\\
in Computer Science 2015 (FICS 2015)\\
EPTCS 191, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.191.3}{10.4204/EPTCS.191.3}}
\pdfoutput=1

